On the dynamics of phase transitions and the nonequilibrium formation of topological defects

We study the formation of topological defects in nonequilibrium phase transitions of both classical and quantum field theory. We examine three model systems. 1). The phase transition of a quantum scalar field in a FRW universe is analyzed through a first-principles approach in which the dynamics of the two-point function is derived from the two-loop, two-particle-irreducible closed-time-path effective action. Identifying signatures of correlated domains in the infrared portion of the momentum-space power spectrum we find that the domain size scales as a power-law with the expansion rate of the universe. The observed power-law scaling is in good agreement with the predictions of the Kibble-Zurek mechanism of defect formation and provides evidence of the freeze-out scenario in the context of nonequilibrium quantum field theory. 2). The formation and interaction of topological textures is analyzed in the phase transition of a classical O(3) scalar field theory in 2+1 dimensions. We provide quantiive arguments that by the end of the transition the length scales of the texture distribution result from a competition between the length scale determined at freeze-out and the ordering dynamics of a textured system. 3). We discuss a black hole phase transition in semiclassical gravity. We review the thermodynamics of a black hole system and determine that the phase transition is entropically driven. We introduce a quantum atomic model of the equilibrium black hole system and show that the phase transition is realized as the abrupt excitation of a high energy state. We investigate the nonequilibrium dynamics of the black hole phase transition and explore similar examples from the Kosterlitz-Thouless transition in condensed matter to the Hagedorn transition in string theory.

==> abstract.tex <==
We study the dynamical formation of topological defects in
nonequilibrium phase transitions of classical and quantum field theory.
We examine three model systems.
{\bf 1)}.~The symmetry-breaking phase transition of a quantum scalar field 
in a Friedmann-Robertson-Walker universe is analyzed through
a first-principles, microscopic approach in which the nonperturbative, nonequilibrium dynamics 
of the two-point function is derived from the two-loop, two-particle-irreducible 
closed-time-path effective action. Identifying signatures of correlated domains in the infrared portion of the 
momentum-space power spectrum we find that the average domain size scales as a power-law with the 
expansion rate of the universe. The observed power-law scaling, for both overdamped and underdamped evolution,  
is in good agreement with the predictions of the Kibble-Zurek mechanism of defect formation 
and provides evidence of the
freeze-out scenario in the context of nonequilibrium quantum field theory.
{\bf 2)}.~The formation and interaction of topological textures is analyzed in the nonequilibrium phase transition
of a classical O(3) scalar field theory in $2+1$ dimensions.  At early times, we observe 
power-law scaling of the length scales of the texture distribution 
in good agreement with the Kibble-Zurek mechanism.  However, the scaling
of the texture distribution changes at late times.  We provide quantitative arguments that by the end 
of the transition the length scales of the texture distribution result from a competition between the 
length scale determined at freeze-out and the ordering dynamics of a textured system.  Therefore, a quantitative
understanding of the defect network at the end of the phase transition requires an understanding of
both critical dynamics {\it and} the interactions among topological defects. 
{\bf 3)}.~We discuss a black hole phase transition in semiclassical gravity. We review the thermodynamics of a black hole system
and determine that the phase transition is entropically driven.
We introduce a quantum atomic model of the equilibrium black hole system and show that the 
phase transition is realized as the abrupt excitation of a high energy state.  
We investigate the nonequilibrium dynamics of 
the black hole phase transition and explore similar examples from the Kosterlitz-Thouless transition in 
condensed matter to the Hagedorn transition in string theory.


==> ack.tex <==
First and foremost I wish to thank my thesis advisor, Prof.~Bei-Lok Hu.  He has been
an unwavering source of patient advice and sound wisdom throughout the Ph.D.~process.  
Through our many discussions and by his own example, Prof.~Hu has taught me
much of what it means to be a theoretical physicist.  As a mentor, he allowed 
me space to find my own creative, scientific voice.  I will always be grateful for 
the intense time we spent together when I was a graduate student and I look forward to many fruitful 
collaborations.

This work was supported in part by NSF grant PHY-9800967.  I thank Prof.~Hu for providing
RA funding and also for partially funding conference appearances in France, Santa Barbara, Seattle
and Brookhaven; all of these provided me with the opportunity to interact with a wide scientific community.
I thank Prof. Esteban Calzetta for his collaboration in part of this research and
for many interesting discussions. 

I benefited enormously from the community of professors, postdoctoral fellows and
graduate students that make up the Maryland Relativity group.  I am lucky to have found
such an environment.
In particular I wish to thank Prof.~Dieter Brill for his support when I first
arrived at Maryland and Prof.~Theodore Jacobson for all of our many discussions.
I would also like to thank Dr.~Charris Anastopolous, Dr.~Phil Johnson, Conrad Schiff
and Prof.~Jonathon Simon for useful advice and encouragement over the years.
I would especially like to thank Dr.~Stephen Ramsey for his collaboration, friendship and
advice (and mountaineering companionship). 

My family provided critical financial and emotional support.  Without them
I never would have made it to graduate school, let alone finished.

Finally I would like to thank Karen, my best friend, who has taught me so much 
about life and whose warm support has kept me sane and balanced.  For her I do the doctor dance.


